Environmental variation of the low-mass IMF

We use a series of magnetohydrodynamic simulations including both radiative and protostellar outflow feedback to study the environmental variation of the initial mass function. The simulations represent a carefully-controlled experiment whereby we keep all dimensionless parameters of the flow constant except for those related to feedback. We show that radiation feedback suppresses the formation of lower mass objects more effectively as the surface density increases, but this only partially compensates for the decreasing Jeans mass in denser environments. Similarly, we find that protostellar outflows are more effective at suppressing the formation of massive stars in higher surface density environments. The combined effect of these two trends is towards an IMF with a lower characteristic mass and a narrower overall mass range in high surface density environments. We discuss the implications of these findings for the interpretation of observational evidence of IMF variation in early-type galaxies.

==> scratch.tex <==
%The differences in the temperatures in the runs are solely



%At the beginning of the simulations, the gas temperature in the simulations are at 10K. As star formation process begins, the gas surrounding the stars begins to heat up. By the time the s 

%In figure 1 we can see star formation has mostly occurred in the dense filamentary regions in these runs. 
%Figure 1 shows the evolution of the


While such a theory can very naturally explain the power-law tail of the IMF, and there is good numerical evidence that turbulence does indeed determine this feature \citep{Nam21a}, apart from the driving and dissipations scales, and the sonic scale \citep{FederrathEtAl2021}, isothermal turbulence is a scale-free process in the ‘inertial range’ (Kolmogorov 1941; Burgers 1948)."



%\subsubsection{Limitations}
%There is a limitation in the methodology we used for radiation transfer. We assume that the gas and dust temperatures are equal. Since the gas and dust temperatures become identical at densities above $\rm 10^{4}-10^{5} cm^{-3}$ \citep[e.g][]{2001ApJ...557..736G}, this is a good assumption for most of the gas in the simulation box. However, in the low density, non-self-gravitating regions, this is not a good assumption since we are overestimating the dust cooling rate of the gas in these regions.




From this plot it is clear that the escape speeds in the low surface density runs are systematically higher than the high surface density runs. This is because stellar evolution takes more physical time than evolution time to reach the same SFE and thus the stars have longer to contract. The higher escape speed also means that more energy is released per unit mass accreted. \autoref{fig:outflow} shows the outflow kinetic energy, momentum and volume relative to the box kinetic energy, momentum and volume. The low surface density runs produce almost three times as much kinetic energy, twice as much momentum and twice as much volume compared to the high surface density runs. This makes it easier for the outflows to punch holes into the collapsing cores in the low surface density runs. This leads to less fragmentation at the high mass end for the low surface density runs and therefore it leads to a heavier IMF.








If there was no feedback in our simulations the stellar mass would scale just like the jeans mass would have scaled which is  



our paper using the current scaling is that if you had no feedback then you would expect to have mean stellar mass just scale like the Jeans mass does, as Sigma^(-1/2), but radiation feedback flattens that a bit, so it winds up being more like Sigma^(-1/3). So suppose we go with this idea. A first thing to calculate then is how the Jeans mass would change with surface density under this alternative scaling where you vary the sound speed rather than the mass in the box. That is the first order answer for how the IMF would change in that scenario. Then you can add the first order perturbation on top of this: all other things being equal, I expect stellar radiation feedback to be more effective in a simulation where the background temperature is lower, just because then it requires less energy input to heat things up compared to the background. So how does that change the initial scaling you got based on the Jeans mass?

Changing the temperature would change the scaling of the jeans mass in the simulations. Radiation feedback and outflow feedback will have similar impact on the simulations same as the simulations presented in this paper with a different peak mass probably.

%where $M_{j} \propto \frac{1}{\sqrt{\rho}}$. 



%But What if, rather than holding $T$ / $c_s$ constant, we instead varied them and held box mass constant? 


%\subsection{Limitations}


%Another thing we do not take into account is the CMB temperature. For all our runs we use a floor temperature of 10K. But as we go up in the redshift to more and more ETG like environments the CMB temperature does add to the floor temperature. In our runs we don't account for that.

%Dust-gas coupling

%CMB









%on a uniform $\rm 512^{3}$ grid. According to \cite{2012ApJ...745..139L}, this resolution is sufficient enough to capture a well-resolved inertial cascade down to the scale of L/30 = 0.02 pc. This scale is one order magnitude less than the initial jeans length in our simulations, so the driving phase produces well-resolved turbulence down to scales well below the scale at which self-gravity is expected to become important.
